PopSim: An Individual-level Population Simulator for Equitable Allocation of City Resources

Historical systematic exclusionary tactics based on race have forced people of certain demographic groups to congregate in specific urban areas. Aside from the ethical aspects of such segregation, these policies have implications for the allocation of urban resources including public transportation, healthcare, and education within the cities. The initial step towards addressing these issues involves conducting an audit to assess the status of equitable resource allocation. However, due to privacy and confidentiality concerns, individual-level data containing demographic information cannot be made publicly available. By leveraging publicly available aggregated demographic statistics data, we introduce PopSim, a system for generating semi-synthetic individual-level population data with demographic information. We use PopSim to generate multiple benchmark datasets for the city of Chicago and conduct extensive statistical evaluations to validate those. We further use our datasets for several case studies that showcase the application of our system for auditing equitable allocation of city resources.

==> anova_results_table.tex <==
\begin{table}[]
\centering
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{ccc}
\hline
\multirow{2}{*}{Datasets} & \multicolumn{2}{c}{One way ANOVA} \\ \cline{2-3} 
                          & Statistic       & p-value         \\ \hline
Schools                   & 18171.5         & 0.000           \\
Hospitals                 & 24049.3         & 0.000       \\
Bus stops                 & 2969.0         & 0.000       \\
L train stations          & 47505.6       & 0.000      \\
Divvy bike stations       & 13843.8          & 0.000     
\end{tabular}%
% }
\caption{Study Case's ANOVA Table}
\label{tab:tabthird}
\end{table}

==> archive/method.tex <==
\section{System Development Details}\label{sec:methods}

Here, we assume that our computer is capable of generating totally independent instances of a random variable $U$ uniformly distributed on $[0,1]$ whenever required. 

In this paper, we will focus on the discrete transform method. Assume that $X$ is a discrete random variable having ${x_1,x_2,..,x_n}$ outcomes such that $P(X=x_i)=p_i \forall 1\le i \le n$. The algorithm is implemented as follows:
\begin{enumerate}
    \item Generate $U\sim Unif(0,1)$.
    \item Determine the index $k$ such that 
    $\sum^{k - 1}_{j=1} p_j\le U< \sum^{k}_{j=1}p_j$, and return $X=x_k$.
\end{enumerate}





\subsection{Sampling Strategy}

The sampling size of the Illinois synthesis population of $n$ individuals  with the number of categorical races of $m = 64$ and number of blocks of $b = 12,006$. For each individual in the synthesis dataset, We must sampling three attributes: the FIPS of the block they reside in, their race, and their GPS location.

\subsubsection{Sampling Block FIPS}

First, we calculate the cumulative distribution function of the total population through blocks for the processed Illinois' Population Dataset. It will return a list of distribution probability $V$ of ${v_1, v_2, ..., v_b}$ such that for every block $b_i$:  

\begin{equation}
v_i = \frac{ \sum_{i = 0}^{t}(v_t)}{\sum_{i = 0}^{b}(v_t)}
\end{equation}

Then, we use the Inverse Transform Sampling method to pick out $n$ $(n = 12,812,508)$ block FIPS samples ${f_1, f_2, ..., f_n}$ from the given cumulative distribution function of the total population for the processed Illinois' Population Dataset.

Then we count the number of occurrences of every FIPS existed in the list ${f_1, f_2, ..., f_n}$, which returns a dictionary of ${z_1:w_1, z_2:w_2,... ,z_k:w_k}$ for each block $z_i$ has $w_i$ people.


\subsubsection{Sampling Person Racial Information}
For each block $z_i$ has $w_i$ people, we calculate the cumulative distribution function of the total population through races using the given block $z_i$'s racial population in Illinois' Population Dataset. It will return a list of distribution $H$ of ${h_1, h_2, ..., h_b}$ such that for every race $h_i$: 
\begin{equation}
h_i =\frac{ \sum_{i = 0}^{t}(h_t)}{\sum_{i = 0}^{m}(h_t)}
\end{equation}

Then, we use the Inverse Transform Sampling method to pick out $w_i$ race samples $R_i$ of ${r_1, r_2, ..., r_{w_i}}$ from the given cumulative distribution function of the total population for the processed Illinois' Population Dataset.

Then we assign each of the person $p_i$ with the race $r_i$.

\subsubsection{Sampling Locations}

For each block $z_i$ has $w_i$ people, we will obtain the boundary region for block $z_i$. Then, we will use the Monte Carlos method for Sampling Random Location in order to pick out $w_i$ random locations. Then we assign each location for each person in $w_i$ people. 
% \begin{center}
% 	\includegraphics[width=8cm, height=5cm]{images/randomize-location-block.png}
% \end{center}

\subsubsection{Monte Carlo's Methods For Sampling Random Locations}
% Monte Carlo techniques, also known as Monte Carlo experiments, are a large category of computing algorithms that depend on repeated random sampling to get numerical results. The core premise is to leverage chance to solve problems that are in essence deterministic. This work focuses on the generation of samples from a given geographical boundary.

% We also follow the pattern of the usual Monte Carlo's Method:

% \begin{enumerate}
%     \item Define a domain of possible inputs.
%     \item Generate inputs randomly from a probability distribution over the domain.
%     \item Perform a deterministic computation on the inputs.
%     \item Aggregate the results.
% \end{enumerate}

Specifically, with given boundary $B$ of a shape $U$, we will generate a set of $T$ containing $n$ points lies within the boundary $B$ by:

\begin{enumerate}
    \item Create an bounding rectangle $R$ of boundary $B$ such that it has the four vertices of $(x_{min}, y_{min})$, $(x_{min}, y_{max})$, $(x_{max}, y_{min})$, $(x_{max}, y_{max})$ where $x_{max}$, $x_{min}$ are the maximum and minimum of boundary's longitudes and $y_{max}$, $y_{min}$ are the maximum and minimum of boundary's latitudes.
    \item We create two uniform distributions of $X\sim U(x_{min}, x_{max})$ and $Y\sim U(y_{min}, y_{max})$.
    \item For a point $P(x_i, y_i)$ with $x_i$ in $X$ and $y_i$ in $Y$, we validate the location of point $P$ whether it is within the boundary $B$.
    \item If point $P$ lies within the boundary $B$, then add point $P$ to set $T$. Otherwise, continue to step 5.
    \item If the set $T$ contains $n$ points, return set $T$. Else, move the step 3.
\end{enumerate} 

